Sampling for Data Freshness Optimization: Non-linear Age Functions

In this paper, we study how to take samples at a data source for improving the freshness of received data samples at a remote receiver. We use non-linear functions of the age of information to measure data freshness, and provide a survey of non-linear age functions and their applications. The sampler design problem is studied to optimize these data freshness metrics, even when there is a sampling rate constraint. This sampling problem is formulated as a constrained Markov decision process (MDP) with a possibly uncountable state space. We present a complete characterization of the optimal solution to this MDP: The optimal sampling policy is a deterministic or randomized threshold policy, where the threshold and the randomization probabilities are characterized based on the optimal objective value of the MDP and the sampling rate constraint. The optimal sampling policy can be computed by bisection search, and the curse of dimensionality is circumvented. These age optimality results hold for (i) general data freshness metrics represented by monotonic functions of the age of information, (ii) general service time distributions of the queueing server, (iii) both continuoustime and discrete-time sampling problems, and (iv) sampling problems both with and without the sampling rate constraint. Numerical results suggest that the optimal sampling policies can be much better than zero-wait sampling and the classic uniform sampling.

==> sec_analysis_1.tex <==
\ifreport



\section{Proof of Theorem \ref{thm1}}\label{sec_analysis}

%In this section, we prove Theorem \ref{thm1} in two steps: 
%%First, we show that given any sampling policy, the MMSE estimation policy \eqref{eq_esti} is optimal for minimizing the objective function in \eqref{eq_DPExpected}. The remaining task is to solve the optimal sampling problem given an MMSE estimator. Second, 
%First, we  show that no sample should be generated when the server is busy, which simplifies the online sampling problem. Second, we use  \cite[Lemma 2]{Sun_reportISIT17} to further simplify the online sampling problem and then use . the  
%
%in  the Lagrangian dual problem of the simplified problem, and decompose the Lagrangian dual problem into a series of \emph{mutually independent} per-sample control problems. Each of these per-sample control problems has a simple solution. Next, we show that the Lagrangian duality gap of our Markov decision problem is zero. By this, Problem \eqref{eq_problem} is solved. The details are as follows.

\subsection{Simplification of Problem \eqref{eq_problem}}

In \cite{AgeOfInfo2016,SunInfocom2016}, it was shown that \emph{no new sample should be taken when the server is busy}. The reason is as follows: If a sample is taken when the server is busy, it has to wait in the queue for its transmission opportunity; meanwhile the sample is becoming stale. A better strategy is to take a new sample once the server becomes idle. By using the sufficient statistic of the Markov chain $X_n$, one can show that the second strategy is better. 

Because of this, we only need to consider a sub-class of sampling policies $\Pi_1\subset\Pi$ in which each sample is generated and submitted to the server after the previous sample is delivered, i.e.,
\begin{align}
\Pi_1 %&= \{\pi\in\Pi: S_{i} = G_{i} \geq D_{j} \text{ for all $i$ and $j=1,\ldots,i$}\} \nonumber \\
 &= \{\pi\in\Pi: S_{i+1} \geq D_{i} = S_i + Y_i \text{ for all $i$}\}. 
\end{align}
Let $Z_i = S_{i+1} -D_{i} \geq0$ represent the waiting time between the delivery time $D_i$ of sample $i$ and the generation time $S_{i+1}$ of sample $i+1$. Since $S_1 = 0$, we have
$S_i =  S_{1} +\sum_{j=1}^{i} (Y_{j} + Z_j)=\sum_{j=1}^{i} (Y_{j} + Z_j)$ and $D_i = S_i + Y_i$. Given $(Y_1,Y_2,\ldots)$, $(S_1,S_2,\ldots)$ is uniquely determined by $(Z_1,Z_2,\ldots)$. Hence, one can also use $\pi = (Z_1,Z_2,\ldots)$ to represent a sampling policy in $\Pi_1$. 



Because $T_i $ is a regenerative process, 
using the renewal theory in \cite{Ross1996} and \cite[Section 6.1]{Haas2002}, one can show that in Problem \eqref{eq_problem}, $\frac{1}{i} 
\mathbb{E}[S_i]$ and $\frac{1}{i} 
\mathbb{E}[D_i]$ are convergent sequences and %$(Z_1,Z_2,\ldots)$ is also stationary and ergodic. Hence, 
%Because  $(Y,Y_2,\ldots)$ are \emph{i.i.d.} and $(Z_1,Z_2,\ldots)$ are stationary and ergodic, we can obtain
\begin{align}
&\limsup_{N\rightarrow \infty}\frac{1}{N}~\mathbb{E}\left[\sum_{n=1}^N p(\age_n)\right] \nonumber
\\
=& \lim_{i\rightarrow \infty}\frac{\mathbb{E}\left[\sum_{n=1}^{D_i} p(\age_n)\right]}{\mathbb{E}[D_i]} \nonumber\\
=& \lim_{i\rightarrow \infty}\frac{\sum_{j=1}^{i}\mathbb{E}\left[\sum_{n=D_{j}}^{D_{j+1}-1}p(\age_n)\right]}{\sum_{j=1}^{i} \mathbb{E}\left[Y_j+Z_j\right]}.\nonumber
%= & \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\right]}{ 6\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]} +  \mathbb{E}\left[Y\right],\nonumber
\end{align}
In addition, for each policy in $\Pi_1$, it holds that $D_i \leq D_{i+1}$. In this case, the age $\age_n$ in \eqref{eq_age} can be expressed as 
\begin{align}
\age_n = n- S_i,~\text{if}~D_i\leq n < D_{i+1}. \nonumber
\end{align}
Hence,
\begin{align}\label{eq_sum1}
\sum_{n=D_{i}}^{D_{i+1}-1}\!\!p(\age_n)=\!\!\sum_{n=D_{i}}^{D_{i+1}-1}\!\!p(n-S_i)=\!\!\sum_{n=Y_{i}}^{Y_i+Z_i+Y_{i+1}-1}\!\!p(n), 
\end{align}
which is a function of $(Y_i,Z_i,Y_{i+1})$. Define 
\begin{align}\label{eq_sum}
q(Y_i,Z_i,Y_{i+1})= \sum_{n=Y_{i}}^{Y_i+Z_i+Y_{i+1}-1}\!\!p(n), 
\end{align}
then  \eqref{eq_problem} can be simplified as 
\begin{align}\label{eq_problem_S1}
\bar p_{\text{opt}} = \inf_{\pi\in\Pi_1}~&\lim_{i\rightarrow \infty}\frac{\sum_{j=1}^{i}\mathbb{E}\left[q(Y_j,Z_j,Y_{j+1})\right]}{\sum_{j=1}^{i} \mathbb{E}\left[Y_j+Z_j\right]}.
%\\
%\text{s.t.}~~& \lim_{i\rightarrow \infty} \frac{1}{i}\sum_{j=1}^{i} \mathbb{E}\left[Y_j+Z_j\right] \geq \frac{1}{f_{\max}}.
\end{align}

In order to solve \eqref{eq_problem_S1}, let us consider the following Markov decision problem with a parameter $c\geq 0$:
%In order to solve \eqref{eq_Simple}, let us consider the following Markov decision with a parameter $c$:
\begin{align}\label{eq_SD}
\!\!h(c)\!\triangleq\!\inf_{\pi\in\Pi_1}&\lim_{i\rightarrow \infty}\frac{1}{i}\sum_{j=0}^{i-1}\mathbb{E}\left[q(Y_j,Z_j,Y_{j+1})-c(Y_j+Z_j)\right]
\!\!\!\!
%\text{s.t.}~&\lim_{i\rightarrow \infty} \frac{1}{i}\sum_{j=1}^{i} \mathbb{E}\left[Y_j+Z_j\right] \geq \frac{1}{f_{\max}},\nonumber
\end{align}
where $h(c)$ is the optimum  value of \eqref{eq_SD}. Similar with Dinkelbach's method  \cite{Dinkelbach67} for nonlinear fractional programming, the following lemma in \cite{Sun_reportISIT17} also holds for our Markov decision problem \eqref{eq_problem_S1}:

\begin{lemma} \label{lem_ratio_to_minus} \cite[Lemma 2]{Sun_reportISIT17}
The following assertions are true:
\begin{itemize}
\item[(a).] \emph{$\bar p_{\text{opt}}  \gtreqqless c $} if and only if $h(c)\gtreqqless 0$. 
\item[(b).] If $h(c)=0$, the solutions to \eqref{eq_problem_S1}
and \eqref{eq_SD} are identical. 
\end{itemize}
\end{lemma}

Hence, the solution to \eqref{eq_problem_S1} can be obtained by solving \eqref{eq_SD} and seeking $\bar p_{\text{opt}}\in\mathbb{R}$  that satisfies
\begin{align}\label{eq_c}
h(\bar p_{\text{opt}})=0. 
\end{align}

\subsection{Optimal Solution of  \eqref{eq_SD} for \emph{$c = \bar p_{\text{opt}}$} }
%Although \eqref{eq_SD} is not a convex optimization problem, it is possible to use the Lagrangian dual approach to solve \eqref{eq_SD} and show that it admits no duality gap. 
%
%When $c = \bar p_{\text{opt}}$, define the following Lagrangian
%\begin{align}\label{eq_Lagrangian}
%& L(\pi;\lambda) \nonumber\\
%=&\lim_{i\rightarrow \infty}\frac{1}{i}\sum_{j=0}^{i-1}\!\mathbb{E}\!\left[q(Y_j,Z_j,Y_{j+1})\!-\! \bar p_{\text{opt}} (Y_j\!+\!Z_j)\right] + \frac{\lambda}{f_{\max}},
%\end{align}
%where $\lambda\geq0$ is the dual variable. 
%Let
%\begin{align}\label{eq_primal}
%g(\lambda) \triangleq \inf_{\pi\in\Pi_1}  L(\pi;\lambda).
%\end{align}
%Then, the Lagrangian dual problem of \eqref{eq_SD} is defined by
%\begin{align}\label{eq_dual}
%d \triangleq \max_{\lambda\geq 0}g(\lambda),
%\end{align}
%where $d$ is the optimum value of \eqref{eq_dual}. 
%Weak duality \cite{Bertsekas2003,Boyd04} implies that $d \leq h(\bar p_{\text{opt}})$. In Section \ref{sec:dual}, we will establish strong duality, i.e., $d = h(\bar p_{\text{opt}})$.

%\subsection{The Optimal Solution to \eqref{eq_primal}}

%We solve \eqref{eq_primal} in several steps: First, we  prove that there exists a \emph{stationary randomized policy} that is optimal for  \eqref{eq_primal}. Next, we prove that there exists a \emph{stationary deterministic policy} that is optimal for  \eqref{eq_primal}. Finally, we find the optimal stationary deterministic policy. 

Next, we present an optimal solution to \eqref{eq_SD} for $c = \bar p_{\text{opt}}$.  

\begin{definition}
A policy $\pi\in\Pi_{1}$ is said to be a \emph{stationary randomized} policy, if it observes $Y_i$ and then chooses a waiting time $Z_i\in[0,\infty)$ 
based on the observed value of $Y_i$, %. Specifically, $Z_i$ is determined 
according to a conditional probability measure $p(y,A)\triangleq\Pr[Z_i\in A| Y_i=y]$ that is invariant for all $i=1,2,\ldots$ Let $\Pi_{\text{SR}}$ ($\Pi_{\text{SR}}\subset \Pi_1$)  denote the set of stationary randomized policies, defined by
\begin{align}
&\Pi_{\text{SR}}\!=\!\{\pi\in\Pi_1: \text{Given the observation $Y_i=y_i$, $Z_i$ is chosen}\nonumber\\
&\text{according to the probability measure } p(y_i,A) \text{ for all } i\}.\nonumber
\end{align}
\end{definition}


%\begin{lemma}\label{lem_SRoptimal} %(Optimality of Stationary Deterministic Policies)
%If the service times $Y_i$ are {i.i.d.}, then there exists a stationary randomized policy that is optimal for solving \eqref{eq_SD} with \emph{$c = \bar p_{\text{opt}}$}.
%\end{lemma}
%\begin{proof}
%%The key proof idea is to show that $Y_i$ is a sufficient statistic for determining $Z_i$ in \eqref{eq_primal}.
%%See Appendix \ref{app2} for the details.
%
%In \eqref{eq_SD}, the minimization of the term 
%\begin{align}\label{eq_opt_stopping1}
%&\mathbb{E}\left[q(Y_j,Z_j,Y_{j+1})- \bar p_{\text{opt}} (Y_j+Z_j)\right]\nonumber\\
%=&\mathbb{E}\left[q(Y_j,Z_j,Y_{j+1})- \bar p_{\text{opt}} (Z_j+Y_{j+1})\right]
%\end{align}
%over $Z_j$ depends on $(Y_1,\ldots,Y_j, Z_1,\ldots,Z_{j-1})$ via $Y_j$. Hence, $Y_j$ is a sufficient statistic for determining $Z_j$ in \eqref{eq_SD}. This means that the rule for determining $Z_i$ can be represented by the conditional probability distribution $\Pr[Z_i\in A| Y_i=y_i]$, and in addition, there exists an optimal  solution $(Z_1,Z_2,\ldots)$ to \eqref{eq_SD}, in which $Z_i$ is determined by solving 
%\begin{align}\label{eq_opt_stopping2}
%\!\!\!\!\min_{\substack{\Pr[Z_i\in A| Y_i=y_i]}} \!\!\!\!\mathbb{E}\left[q(Y_i,Z_i,Y_{i+1})\!-\! \bar p_{\text{opt}} (Z_j+Y_{j+1})\big|Y_i=y_i \right]\!,\!\!
%\end{align}
%and then use  the observation $Y_i=y_i$ and the optimal conditional probability distribution $\Pr[Z_i\in A| Y_i=y_i]$ that solves \eqref{eq_opt_stopping2}  to decide $Z_i$. Finally, notice that the minimizer of \eqref{eq_opt_stopping2} depends on the joint distribution of $Y_i$ and $Y_{i+1}$. Because the $Y_i$'s are  \emph{i.i.d.},  the joint distribution of $Y_i$ and $Y_{i+1}$ is invariant for $i=1,2,\ldots$ Hence, the optimal conditional probability measure $\Pr[Z_i\in A| Y_i=y_i]$ solving \eqref{eq_opt_stopping2} is invariant for $i=1,2,\ldots$ By definition,  there exists a stationary randomized policy that is optimal for solving Problem \eqref{eq_SD} with $c = \bar p_{\text{opt}}$, which completes the proof.
%\end{proof}



%In the sequel, when we refer to the stationary distribution of a stationary randomized policy $\pi\in \Pi_{\text{SR}}$, we will remove  subscript $i$. In particular, {the random variables $(Y_i,Z_i,Y_{i+1})$ are replaced by $(Y,Z,Y')$}, where $Z\geq0$ is chosen based on the conditional probability measure $\Pr[Z\in A| Y=y] =p(y,A)$ after observing $Y=y$, $Y$ and $Y'$ are \emph{i.i.d.} random variables with the same joint distribution as $Y_i$. 
%By Theorem \ref{lem_SRoptimal}, problem \eqref{eq_primal} can be simplified as
%\begin{align}\label{eq_opt_stopping3}
%\min_{p(y,A)} \mathbb{E}\left[q(Y,Z,Y')\!-\! \bar p_{\text{opt}} (Y+Z)\big|Y \right],
%\end{align}
% where $p(y,A) = \Pr[Z\in A| Y=y]$ is the conditional probability measure corresponding to  a stationary randomized policy. 
Next, by using an idea similar to that in the solution of \cite[Problem 5.5.3]{Bertsekas}, we can obtain 
%the solution to \eqref{eq_opt_stopping2} can be obtained as 
% we can obtain
\begin{lemma}\label{lem4}
If $p: \mathbb{R}\mapsto \mathbb{R}$ is non-decreasing and the service times $Y_i$ are {i.i.d.}, then an optimal solution $(Z_1,Z_2,\ldots)$ of \eqref{eq_SD} is given by
%for any given observation $Y=y$, the optimal $Z$ in \eqref{eq_opt_stopping3} is determined by
\begin{align}\label{lem4_eq1}
Z_i = \min\{n\in \mathbb{N}: \mathbb{E}\!\left[p(Y_i+n+Y_{i+1})|Y_i\right]\! \geq\! \beta \},
\end{align}
where \emph{$\beta = \bar p_{\text{opt}}$}.
\end{lemma}
\begin{proof}
%See Appendix \ref{app3}.
Using \eqref{eq_sum} and $\beta = \bar p_{\text{opt}} $, \eqref{eq_opt_stopping2} can be expressed as
\begin{align}\label{eq_opt_stopping4}
\min_{\substack{\Pr[Z_i\in A| Y_i=y_i]}} \mathbb{E}\left[\sum_{n=0}^{Z_i+Y_{i+1}-1}\!\![p(n+Y_i)- \beta] \Bigg| Y_i\right].
\end{align}
It holds that  for $m =1, 2,3,\ldots$
\begin{align}\label{eq_opt_stopping5}
&\mathbb{E}\!\!\left[\sum_{n=0}^{m+Y_{i+1}}\!\!\!\![p(n+Y_i)- \beta] -\!\!\sum_{n=0}^{m+Y_{i+1}-1}\!\!\!\![p(n+Y_i)- \beta] \Bigg| Y_i\right]\nonumber\\
=& \mathbb{E}\!\left[p(Y_i+m+Y_{i+1})- \beta|Y_i\right].
\end{align}
Because $p: \mathbb{R}\mapsto \mathbb{R}$ is non-decreasing, if $Z_i$ is chosen according to  \eqref{lem4_eq1}, we can obtain
\begin{align}
&\mathbb{E}\!\left[p(Y_i+n+Y_{i+1})-\beta |Y_i\right] < 0,~ n = 0, \ldots,  Z_i-1, \\
&\mathbb{E}\!\left[p(Y_i+n+Y_{i+1})-\beta |Y_i\right] \geq 0,~ n \geq Z_i.\label{eq_opt_stopping6}
\end{align}
Based on \eqref{eq_opt_stopping5}-\eqref{eq_opt_stopping6}, it is easy to see that \eqref{lem4_eq1} is the optimal solution to \eqref{eq_opt_stopping4}. 
This completes the proof.
\end{proof}

%\subsection{Zero Duality Gap between \eqref{eq_SD} and \eqref{eq_dual}} \label{sec:dual}
%
%
%Similar to Theorem 7 in \cite{Sun_reportISIT17}, strong duality can be established in the following lemma:
%\begin{lemma}\label{thm_zero_gap}
%If \emph{$c= \bar p_{\text{opt}}$}, the following assertions are true:
%\begin{itemize}
%\vspace{0.5em}
%\item[(a).] The duality gap between \eqref{eq_SD} and \eqref{eq_dual} is zero, i.e., \emph{$d = h(\bar p_{\text{opt}})$}.
%\vspace{0.5em}
%\item[(b).] A common optimal solution to \eqref{eq_problem},  \eqref{eq_problem_S1}, and \eqref{eq_SD} is given by \eqref{thm1_eq4}, \eqref{thm1_eq5}, and \eqref{lem4_eq1}. The optimal value of \eqref{eq_problem} is given by \eqref{thm1_eq3}.
%\end{itemize}
%%Hence, the MMSE-optimal  policy in \eqref{eq_opt_solution} and \eqref{eq_thm1} is an optimal solution to \eqref{eq_SD}. 
%\end{lemma}
%
%\begin{proof}
%The key proof idea is to show that \eqref{eq_SD} has a \emph{geometric multiplier} \cite[Definition 6.1.1]{Bertsekas2003}.\footnote{Note that geometric multiplier is   different from the traditional Lagrangian multiplier.} According to \cite[Proposition 6.2.3]{Bertsekas2003}, if the set of geometric multipliers is non-empty, then the duality gap must be zero, no matter for convex or non-convex optimization problems. 
%The proof details are provided in Appendix \ref{app4}.
%\end{proof}

Hence, Theorem~\ref{thm1} follows from Lemma \ref{lem_ratio_to_minus} and Lemma \ref{lem4}.










==> sec_mutual_info.tex <==
\section{Optimal Sampling for Markov Sources}\label{sec_Markov}
In order to evaluate the the mutual information $I(X_t; \bm{W}_t)=u(\age_t)$, two examples of Markov sources will be discussed in Section \ref{sec_Markov}. 

Two examples of the Markov source $X_t$ are provided in the sequel as illustrations of Lemma \ref{lem1}:
\subsubsection{Gaussian Markov Source} Suppose that $X_t$ is a first-order discrete-time Gaussian Markov process, defined by 
\begin{align}
X_t = a X_{t-1} + Z_t,
\end{align} 
where $a\in(-1,1)$ and the $Z_t$'s are zero-mean \emph{i.i.d.}~Gaussian random variables with variance $\sigma^2$. Because $X_t$ is a Gaussian Markov process, one can show that \cite{Gelfand1959}
\begin{align}
I(X_t; \bm{W}_t) = I\left(X_t; X_{t-\age_t}\right) = -\frac{1}{2} \log_2 \left(1-a^{2\age_t}\right).
\end{align} 
Since $a\in(-1,1)$ and $\age_t\geq 0$ is an integer, $I(X_t; \bm{W}_t)$ is a positive and decreasing function of the age $\age_t$. Note that if $\age_t=0$, then $I(X_t; \bm{W}_t)=H(X_t)=\infty$, because the absolute entropy of a Gaussian random variable is infinite. 
\subsubsection{Binary Markov Source} Suppose that $X_t\in\{0,1\}$ is a binary symmetric Markov chain defined by
\begin{align}\label{eq_binary}
X_t = X_{t-1} \oplus V_t,
\end{align} 
where $\oplus$ denotes binary modulo-2 addition and the $V_t$'s are \emph{i.i.d.} Bernoulli random variables with mean $q\in[0,\frac{1}{2}]$. One can show that
\begin{align}
I(X_t; \bm{W}_t) &= I\left(X_t; X_{t-\age_t}\right) = 1\!-\!h\!\left(\frac{1-(1-2q)^{\age_t} }{2}\right)\!,
\end{align} 
where $\Pr[X_t =1 | X_0=0] = \frac{1-(1-2q)^{n} }{2}$ and $h(x)$ is the binary entropy function defined by $h(x)=-x\log_2 x - (1-x) \log_2 (1-x)$
with a domain $x\in[0,1]$ \cite[Eq. (2.5)]{Cover}. Because $h(x)$ is increasing on $[0,\frac{1}{2}]$, $I(X_t; \bm{W}_t)$ is a not-negative and decreasing function of the age $\age_t$.



\section{Online Sampling for Information Freshness}
In this section, we will develop an optimal online sampling policy that can maximize the freshness of information about Markov sources. 
\subsection{Problem Formulation}

To optimize the freshness of information, we formulate an online sampling problem for maximizing the time-average expected mutual information between $X_t$ and $\bm{W}_t$ over an infinite time-horizon:
\vspace{-0mm}
\begin{equation}\label{eq_problem1}
\bar I_{\text{opt}}=\sup_{\pi\in\Pi}~\liminf_{N\rightarrow \infty}\frac{1}{N}~\mathbb{E}\left[\sum_{t=1}^NI(X_t; \bm{W}_t)\right],
\vspace{-0mm}
\end{equation}
where $\bar I_{\text{opt}}$ is the optimal value of \eqref{eq_problem1}. We assume that $\bar I_{\text{opt}}$ is finite.


It is helpful to remark that $\bar I_{\text{opt}}$ in \eqref{eq_problem1} is different from the Shannon capacity considered in, e.g., \cite{Anantharam1996,Cover}:
In \eqref{eq_problem1}, 
%the received data $\bm{W}_t$ is used to , and 
our goal is to maximize \emph{the freshness of information} and make more accurate inference about the real-time source value; this goal is achieved by minimizing the average amount of mutual information that is lost as the received data becomes obsolete. 
On the other hand, the focus of Shannon capacity theory is mainly on maximizing \emph{the rate of information} that can be reliably transmitted to the receiver, but (in most cases) without significant concerns about whether the received information is new or old. %We will further explore the relationship between the freshness and rate of information in our future work. 


